NeuralCubes: Deep Representations for Visual Data Exploration

Visual exploration of large multidimensional datasets has seen tremendous progress in recent years, allowing users to express rich data queries that produce informative visual summaries, all in real time. Techniques based on data cubes are some of the most promising approaches. However, these techniques usually require a large memory footprint for large datasets. To tackle this problem, we present NeuralCubes: neural networks that predict results for aggregate queries, similar to data cubes. NeuralCubes learns a function that takes as input a given query, for instance, a geographic region and temporal interval, and outputs the result of the query. The learned function serves as a real-time, low-memory approximator for aggregation queries. NeuralCubes models are small enough to be sent to the client side (e.g. the web browser for a web-based application) for evaluation, enabling data exploration of large datasets without database/network connection. We demonstrate the effectiveness of NeuralCubes through extensive experiments on a variety of datasets and discuss how NeuralCubes opens up opportunities for new types of visualization and interaction.

==> Makefile <==
# --------------------------------------------------------------------
# Usage:
#
#	all	 make pdf file
#	pdf	 make pdf file
#	clean	 remove files
#	clobber  remove everything
#	check	 doubled word and latex syntax check
#	wc	 word count
# --------------------------------------------------------------------

NAME := paper
BIBFILES := ref.bib

DISTILLER := ps2pdf

# --------------------------------------------------------------------

SHELL := bash
LATEX := pdflatex
BIBTEX := bibtex -min-crossrefs=100 # avoid separating out crossrefs
DETEX := detex -n
LACHECK := lacheck
DW := dw # ftp://ftp.math.utah.edu/pub/misc/dw.tar.gz
RM := rm -f
WC := wc

# --------------------------------------------------------------------

all: $(NAME).pdf 
pdf: $(NAME).pdf
check: dw syn

draft: $(NAME).tex $(BIBFILES)
	@echo '-------------------- latex #1 --------------------'
	$(LATEX) -draftmode $(NAME).tex
	@echo '-------------------- bibtex --------------------'
	$(BIBTEX) $(NAME)
	@echo '-------------------- latex #2 --------------------'
	$(LATEX) -draftmode $(NAME).tex
	@echo '-------------------- latex #3 --------------------'
	$(LATEX) -draftmode $(NAME).tex


$(NAME).pdf: $(NAME).tex $(BIBFILES)
	@echo '-------------------- latex #1 --------------------'
	$(LATEX) $(NAME).tex
	@echo '-------------------- bibtex --------------------'
	$(BIBTEX) $(NAME)
	@echo '-------------------- latex #2 --------------------'
	$(LATEX) $(NAME).tex
	@echo '-------------------- latex #3 --------------------'
	$(LATEX) $(NAME).tex

dw:
	@-$(RM) $(NAME).dw
	@echo '-------------------- doubled words --------------------'
	@for f in $(NAME).tex ;\
	do \
		echo ----- $$f ----- ; \
		echo ----- $$f ----- >> $(NAME).dw ; \
		$(DETEX) $$f  | $(DW) >> $(NAME).dw ; \
	done

syn:
	@echo '-------------------- syntax check --------------------'
	@$(LACHECK) $(NAME).tex

wc:
	@$(DETEX) $(NAME).tex | $(WC)

jpg:
	./make_jpg.sh

small:
	@echo '-------------------- make jpg --------------------'
	cat paper.tex | sed 's/.png/.jpg/g' > $(NAME)_jpg.tex
	@echo '-------------------- latex #1 --------------------'
	$(LATEX) $(NAME)_jpg.tex
	@echo '-------------------- bibtex --------------------'
	$(BIBTEX) $(NAME)_jpg
	@echo '-------------------- latex #2 --------------------'
	$(LATEX) $(NAME)_jpg.tex
	@echo '-------------------- latex #3 --------------------'
	$(LATEX) $(NAME)_jpg.tex
	cp $(NAME)_jpg.pdf nanocubes_jpg.pdf

notation:
	pandoc notation.md -s --webtex -o notation.pdf
	open notation.pdf

clean:
	$(RM) *.{blg,dvi,dw,ilg,log,o,tmp,lbl,aux,bbl,idx,ind,toc,lof,lot,brf} paper.pdf

clobber: clean
	$(RM) *~ \#* core

